Quantifying the presence of graffiti in urban environments

Graffiti is a common phenomenon in urban scenarios. Differently from urban art, graffiti tagging is a vandalism act and many local governments are putting great effort to combat it. The graffiti map of a region can be a very useful resource because it may allow one to potentially combat vandalism in locations with high level of graffiti and also to cleanup saturated regions to discourage future acts. There is currently no automatic way of obtaining a graffiti map of a region and it is obtained by manual inspection by the police or by popular participation. In this sense, we describe an ongoing work where we propose an automatic way of obtaining a graffiti map of a neighbourhood. It consists of the systematic collection of street view images followed by the identification of graffiti tags in the collected dataset and finally, in the calculation of the proposed graffiti level of that location. We validate the proposed method by evaluating the geographical distribution of graffiti in a city known to have high concentration of graffiti -- Sao Paulo, Brazil.

==> abstract.tex <==
\begin{abstract}

Graffiti is a common phenomenon in urban scenarios. Differently from urban art, graffiti tagging is a vandalism act and many local governments are putting great effort to combat it. The graffiti map of a region can be a very useful resource because it may allow one to potentially combat vandalism in locations with high level of graffiti and also to cleanup saturated regions to discourage future acts. There is currently no automatic way of obtaining a graffiti map of a region and it is obtained by manual inspection by the police or by popular participation. In this sense, we describe an ongoing work where we propose an automatic way of obtaining a graffiti map of a neighbourhood. It consists of the systematic collection of street view images followed by the identification of graffiti tags in the collected dataset and finally, in the calculation of the proposed \emph{graffiti level} of that location. We validate the proposed method by  evaluating the geographical distribution of graffiti in a city known to have high concentration of graffiti -- São Paulo, Brazil.

\end{abstract}


==> acknowledgments.tex <==
\section*{Acknowledgments}

%TODO: modify here later
To be included after approval.
% The authors would like to thank
% FAPESP grants \#2014/24918-0, \#2015/22308-2, CNPq, CAPES and NAP eScience - PRP - USP.

==> conclusion.tex <==

% ##################### Conclusion
\section{Conclusion}

This work presents an ongoing work on automatic mapping of regions containing graffiti tags. We systematically collect street view imagery from~\cite{googlemaps} and identify the graffiti tags in each image and we propose a metric for the graffiti level of a geographical region. We did a case study in São Paulo and show that it is in accordance to what is expected given the indicators of HDI.

There are limitations of the proposed approach. One of them is the requirement of sampling, due to computing constraints. Small regions with highly concentrated tagging do not properly contribute to the metric of the region. An additional point of improvement is the utilization of new vision algorithm with higher performance. Future steps include the test and comparison with other vision algorithms and future steps include a denser sampling and the a joint analysis with other geographical regions.

\begin{figure}[ht]
    \centering
    \subfloat[Coverage]{
        \includegraphics[width=0.15\textwidth]{coverage.pdf} 
 }%
    \qquad
    \subfloat[IDH]{
	\includegraphics[width=0.15\textwidth]{img/idhperdistrict_purple.pdf} 
    }%
    \caption{Coverage our the utilized images using \cite{googlemaps} images. São Paulo districts 2007 HDI. Data from~\cite{atlas2012idh}.}
    \label{fig:metadata}%
\end{figure}

==> experiments.tex <==
\section{Experiments}

%############################## Acquisition
%Google Street View api
% https://www.google.com/permissions/geoguidelines/attr-guide.html
%TODO: CITE above!

We initially collected a pilot sample of 10,000 street view images from~\cite{googlemaps} from São Paulo City and a sample was manually chosen. The regions containing graffiti tags were manually identified. A total 632 of images were manually annotated and used to train Resnet 101-layers backbone~\cite{he2016deep} pre-trained on the Coco dataset~\cite{lin2014microsoft}. We used a learning rate of 0.001 and a momentum of 0.9 and trained for 80 epochs. We used the model obtained in epoch 30, given its highest validation error (see Figure~\ref{fig:losses}). The final model showed an average precision~\cite{everingham2010pascal} of $0.57$. Figure~\ref{fig:detections} presents a sample of the detections evaluated. The full time to process a single image is of $0.69$s on a Geforce GTX 1050.


\begin{figure}[h]
	\centering
	\includegraphics[width=0.45\textwidth]{img/trainvalloss.pdf} 
	\caption{Training and validation loss of the model~\cite{he2017mask} during the training stage.}
	\label{fig:losses}
\end{figure}


In Figure~\ref{fig:metadata}~(a) we can see the heterogeneous coverage of the service utilized~\cite{googlemaps} street view images in the city. The two bottommost districts showed little coverage at the time of our acquisition, given the predominantly rural and unpopulated nature of these regions and thus they were not considered in this study.

%\begin{figure}%
%    \centering
%    \subfloat[Coverage]{
%        \includegraphics[width=0.15\textwidth]{coverage.pdf} 
% }%
%    \qquad
%    \subfloat[IDH]{
%	\includegraphics[width=0.15\textwidth]{img/idhperdistrict_purple.pdf} 
%    }%
%    \caption{Coverage our the utilized images using \cite{googlemaps} images. São Paulo districts 2007 HDI. Data from~\cite{atlas2012idh}.}
%    \label{fig:metadata}%
%\end{figure}



%\begin{figure}[h]
%	\centering
%        \includegraphics[width=0.15\textwidth]{coverage.pdf} 
%	\caption{Coverage our our sample using \cite{googlemaps} images.}
%        \label{fig:coverage}
%%	\includegraphics[width=0.15\textwidth]{img/idhperdistrict_purple.pdf} 
%%	\caption{Human development indices (2007) of São Paulo districts. Data from~\cite{atlas2012idh}.}
%%	\label{fig:hdi}
%\end{figure}

We used four views for each geographical location, spaced by $90^{\circ}$. Notice in Figure~\ref{fig:views} how the scene elements from the second and the third figures intersect which indicates a full coverage for each geographical location. The majority of the images considered are from 2017 as can be seen in Table~\ref{tab:years}. 

\begin{figure}[h]
%\begin{table*}[ht]
%\begin{table}[ht]
\centering
\begin{tabular}{ccc}
	%\includegraphics[width=0.23\textwidth]{{detections/_-23.55229300_-46.50119900_180}.jpg}  &
	%\includegraphics[width=0.23\textwidth]{{detections/_-23.60929300_-46.47319900_270}.jpg}  &
	%\includegraphics[width=0.23\textwidth]{{detections/_-23.61429300_-46.49619900_180}.jpg} \\
	\includegraphics[width=0.23\textwidth]{{detections/_-23.51429300_-46.38619900_90}.jpg} &
	%\includegraphics[width=0.23\textwidth]{{detections/im_-23.54478399999999_-46.64192499999999_240}.jpg}  &
	\includegraphics[width=0.23\textwidth]{{detections/_-23.69229300_-46.66419900_180}.jpg} 
\end{tabular}
\caption{Sample of the graffiti detections. The values depicted represent the confidence of the detections.}
\label{fig:detections}
%\end{table}
%\end{table*}
\end{figure}
%\begin{figure}[h]
        %\centering
        %\includegraphics[width=0.11\textwidth]{_-235424736_-466441269_0.jpg} 
        %\includegraphics[width=0.11\textwidth]{_-235424736_-466441269_90.jpg} 
        %\includegraphics[width=0.11\textwidth]{_-235424736_-466441269_180.jpg} 
        %\includegraphics[width=0.11\textwidth]{_-235424736_-466441269_270.jpg} 
        %\caption{Four views from the same geographical point. }
        %\label{fig:views}
%\end{figure}


\begin{table}[h]
	\centering
	\setlength\tabcolsep{2pt} % default value: 6pt

	\caption{Acquisition year of the geographical location analyzed. Metadata provided by~\cite{googlemaps}.}
	\begin{tabular}{lccccccccc}
		\toprule
		\textbf{Year}&2010 &2011 &2012 &2013 &2014 &2015 &2016 &2017 &2018 \\
		\midrule

		\textbf{Points}&1,241 &16,311 &207 &422 &2,182 &4,563 &4,211 &39,391 &317 \\
		\bottomrule
	\end{tabular}
	\label{tab:years}
\end{table}
We created a grid over the spatial extent of the city with 134,624 points with 102m vertical and horizontal spacing of our grid. After eliminating images from third-party providers and non-mapped regions (see Figure~\ref{fig:metadata})~a, we obtained a geographical coverage of 68,752 geographical points and 275,339 images overall.


%\begin{table}[h]
	%\centering
	%\setlength\tabcolsep{2pt} % default value: 6pt
	%\caption{Number of images per district.}
	%\begin{tabular}{ll}
		%\toprule
		%Grajau&1612\\
		%Tremembe&1413\\
		%Cid dutra&1343\\
		%Jd sao luis&1225\\
		%Itaquera&1196\\
		%Jaragua&1157\\
		%Sapopemba&1153\\
		%Jabaquara&1151\\
		%Capao redondo&1137\\
		%Santo amaro&1134\\
		%Pirituba&1112\\
		%Sacoma&1098\\
		%Cid ademar&1051\\
		%Sao mateus&1034\\
		%Itaim paulista&1022\\
		%Campo limpo&994\\
		%Jd angela&969\\
		%Penha&964\\
		%Vila maria&936\\
		%Brasilandia&919\\
		%Santana&908\\
		%Freguesia do o&884\\
		%Butanta&884\\
		%Morumbi&874\\
		%Ipiranga&845\\
		%Itaim bibi&828\\
		%Cangaiba&818\\
		%Saude&806\\
		%Vila curuca&802\\
		%Cid tiradentes&796\\
		%Iguatemi&793\\
		%Lapa&786\\
		%Campo grande&781\\
		%Sao lucas&780\\
		%Rio pequeno&766\\
		%Cid lider&757\\
		%Vila matilde&756\\
		%Vila prudente&755\\
		%Pedreira&746\\
		%Cursino&746\\
		%Vila mariana&745\\
		%Lajeado&742\\
		%Moema&728\\
		%Vila sonia&728\\
		%Vila jacui&721\\
		%Parelheiros&717\\
		%Anhanguera&704\\
		%Jose bonifacio&699\\
		%Tucuruvi&697\\
		%Pinheiros&691\\
		%Sao domingos&686\\
		%Tatuape&678\\
		%Jacana&662\\
		%Perus&662\\
		%Vila medeiros&644\\
		%Agua rasa&643\\
		%Campo belo&637\\
		%Parque do carmo&632\\
		%Cachoeirinha&632\\
		%Ermelino matarazzo&626\\
		%Sao rafael&626\\
		%Carrao&625\\
		%Vila formosa&619\\
		%Mandaqui&615\\
		%Casa verde&613\\
		%Vila andrade&612\\
		%Sao miguel&609\\
		%Aricanduva&604\\
		%Jd helena&602\\
		%Mooca&594\\
		%Raposo tavares&593\\
		%Ponte rasa&589\\
		%Socorro&586\\
		%Alto de pinheiros&573\\
		%Guaianases&570\\
		%Limao&546\\
		%Perdizes&542\\
		%Artur alvim&539\\
		%Vila guilherme&534\\
		%Jd paulista&502\\
		%Vila leopoldina&449\\
		%Jaguare&410\\
		%Belem&410\\
		%Barra funda&386\\
		%Consolacao&324\\
		%Bom retiro&317\\
		%Jaguara&316\\
		%Santa cecilia&314\\
		%Cambuci&289\\
		%Liberdade&287\\
		%Bras&285\\
		%Bela vista&233\\
		%Pari&220\\
		%Republica&212\\
		%Se&198\\
		%Marsilac&4\\
		%\bottomrule
	%\end{tabular}
	%\label{tab:years}
%\end{table}

%\begin{figure}[ht]
        %\centering
        %\includegraphics[width=0.45\textwidth]{20180622-spcity_capturedon_gray.pdf} 
        %\caption{Capture dates.}
        %\label{fig:dates}
%\end{figure}

%We trained for 80 epochs but utilized the model obtained in epoch 30, given the minimum value of validation loss (see Figure~\ref{fig:losses}.


\begin{figure}[h]
        \centering
        %\includegraphics[width=0.22\textwidth]{img/idhperdistrict_purple.pdf} 
        \includegraphics[width=0.35\textwidth]{img/perdistrict_avgmaskarea_withinvalid_colorbar.png} 
	\caption{Relative graffiti level in São Paulo city. The divisions represent the city districts and the colors in logarithmic scale express the relative graffiti level, according to~(\ref{eq:perregion}). Bottonmost regions were not considered given the unavailability of data in the region.}
        \label{fig:graffitimap}
\end{figure}

We can see in Figure~\ref{fig:graffitimap} that except a small region inside the map, the regions with highest levels of graffiti are in peripheral regions of the city. The regions with lowest levels of graffiti are in the business center of the city. The bottommost parts were not considered given the coverage of the service utilized.

The Human Development Index (HDI) is a \emph{development} measure of a region that considers life span, income and education aspects~\cite{hdr1990concept}. Figure~\ref{fig:metadata}~b is a HDI heat-map by districts using the data released by the city hall~\cite{atlas2012idh} in 2007. Notice that the regions with the lowest levels of graffiti in Figure~\ref{fig:graffitimap} correspond to the regions of highest HDIs in Figure~\ref{fig:metadata}~b.


%\begin{figure}[ht]
%	\centering
%	\includegraphics[width=0.15\textwidth]{img/idhperdistrict_purple.pdf} 
%	\caption{Human development indices (2007) of São Paulo districts. Data from~\cite{atlas2012idh}.}
%	\label{fig:hdi}
%\end{figure}

%##############################


==> introduction.tex <==
\section{Introduction}

Graffiti is already part of the current landscape of most megacities. It can be categorized as artistic drawings or tagging (see Figure~\ref{fig:grafftypes}) and  whereas graffiti drawing is an artistic expression and as such, requires talent and practice, most of the times graffiti tagging represents an unauthorized act that people convey messages or show their names. The discussion whether graffiti is an art is extensively explored~\cite{mcauliffe2012graffiti,young2013street}. In 2017 a Brooklyn based company was fined 6.7 million dollars for whitewashing the murals containing famous graffiti~\footnote{https://www.nytimes.com/2018/02/12/nyregion/5pointz-graffiti-judgment.html}. In this study we focus on the latter and refer to it as simply graffiti. 
  %Studies reveal that there is a strong correlation of people that perform these acts and future criminals~\cite{taylor2012patterns}.
%and major cities combat these acts.

%São Paulo is big city with an estimated GDP of $U\$580$ billion being the richest and a most influential city in South America. There is a high variability in ethnicity and with social levels, which contribute to form a multi-cultural city. Graffiti tagging is spread throughout the city~\cite{theguardian2016pixacao}.

\begin{figure}[ht]
\centering
\begin{tabular}{cc}
\subfloat{\includegraphics[width=0.2\textwidth]{img/im_-23_5563262_-46_6865027_160_shadow.jpg}} &
\subfloat{\includegraphics[width=0.2\textwidth]{img/im_-23_5143383_-46_5711341_0_shadow.jpg}}
\end{tabular}
	\caption{Different types of graffiti . The wall on the left was artistically painted and as such required techniques and time whereas the one on the right is simpler and is composed of words and tags. We are particularly interested in the graffiti type on the right. Images from~\cite{googlemaps}.}
\label{fig:grafftypes}
\end{figure}

There is no São Paulo map of graffiti to our knowledge and creating in by manual inspection would demand great effort. In this work we propose the creation of a graffiti map based on the segmentation of graffiti regions on street view images~\cite{googlemaps}.

Our contribution can be summarized as the proposal of an automated way to quantify the level of graffiti in a location. For this task, street view images are systematically acquired, computer vision algorithms identify and quantify the amount of graffiti in a picture and finally a new metric, the \emph{graffiti level} of the region is devised and computed. We perform a case study in a highly urbanized city, São Paulo, Brazil


% ##########################################################
\section{Related Work}

%There are many initiatives on the combat of graffiti.
%and also several works on image segmentation algorithms and on the use of street view imagery for urban analysis.



%We differ urban art by graffiti tags (see Figure~\ref{fig:grafftypes}).
%  “City, State Abbreviation.” Map. Google Maps. Google, 15 May 2008. Web. 15 May 2008.  

% ##################### Related work
% Patterns of graffiti offending: Towards recognition that graffiti offending is more than ‘kids messing around
%Graffiti writing is primarily an adolescent action and as such, has always been seen as a low-level crime ~\cite{taylor2012patterns}. However, according to~\cite{taylor2012patterns} there is a trend of felonies commited by graffiti writers, not only in terms of types of crimes commited, but also in the frequency of the crimes.

%Cost
%The Australian government estimates a total cost of \$833 million Australian dollars to repair vandalism and graffiti acts in 2011 ~\cite{smith2014counting}.

% Graffiti as art

%There are many initiatives on the combat of graffiti.
There are several works aimed to combat graffiti vandalism acts. Web-based frameworks~\cite{graffititracker,tagrs,graffititracking,vandaltrack} rely on community participation to identify new locations containing graffiti while some works~\cite{angiati2005novel,di2008graffiti, tombari2008graffiti} try to identify the drawing act. Other works retrieve similar graffitis in a reference database~\cite{yang2012efficient} by using connected components and keypoints matching in an attempt to associate graffiti with gangs. Alternatively, ~\cite{tong2011gang} attempts to identify the authorship, given a target image, they compute a metric based on the symbols contained, manually annotate and do a keypoints matching between the images and the gang graffitis.

%graffolution
As a signal of the relevance of the topic, the European Union has a dedicated project~\cite{synyo2016graffolution} to analyze the main actors involved in the graffiti acts, including writers, citizens, law enforcement and public administration. This project includes the consultation of stakeholders and the establishing of a web-based platform that allows the discussion and sharing of ideas about the topic from different perspectives. A number of places alternatively apply more radical measures against these acts~\cite{iveson2010wars}.

% In Brazil, highly densed cities such as São Paulo also face the widespread presence of graffiti in the city~\cite{theguardian2016pixacao}.

%Image retrieval.
%Image retrieval using Sift~\cite{jain2009graffiti}.
%Identify in a fast way spatial and temporal change to identify the act of vandalism using multiple cameras~\cite{di2008graffiti, tombari2008graffiti}

%São Paulo is the richest and a very influential city in Brazil~\cite{ibge2016produto}. The city presents high social unequality which contributes to the widespread presence of graffiti~\cite{theguardian2016pixacao}.

Semantic segmentation is a high-level computer vision task which aims to split the image into known classes~\cite{arbelaez2012semantic}. It is a complex task when compared to image classification and object detection because it requires the image pixel-wise classification. Research on semantic segmentation is very active and recent works achieve impressive results~\cite{arbelaez2012semantic,ronneberger2015u,badrinarayanan2015segnet,zhou2017scene,long2015fully}. A related task is the \emph{instance segmentation}, where the objective is also to identify the instances but in contrast to the ordinary segmentation, the method must be able to identify the boundaries of two adjacents instances. Some previous works~\cite{pinheiro2015learning,dai2016instance} perfomed this task by preceding the object detection stage with a segmentation stage. The work of Mask-RCNN~\cite{he2017mask} in turn performed this task by running the classification and the segment proposals in a parallel manner. \cite{he2017mask} relies on Faster-RCNN~\cite{ren2015faster} architecture but with an additional branch for instance segmentation.

Google Maps\cite{googlemaps} provides public access to images captured by cars driven down the streets. Images are obtained from different geographical locations and in different views and formats. Many works~\cite{rundle2011using,torii2009google} have already utilized this type of imagery for urban analyzes.  The authors of~\cite{doersch2012makes} use street view images to compare the architectural elements from different cities. In~\cite{rundle2011using}, a study on the feasibility on audits of neighbourhoods environments instead of in-person auditing is presented. The work~\cite{li2015assessing} proposes the assessment of urban greenery using the same kind of images.

%There is a high variability in ethnicity and social levels, which contribute to form a multi-cultural city. These facts contribute to the presence of graffiti tagging throughout the city~\cite{theguardian2016pixacao}.

%Aside from fame, visibility and adrenaline, the most important motivation for pixadores is anger – primarily directed against the city. Unlike graffiti (which many pixadores reject as being “too commercial” and a “beautification scheme”), pixação seeks to positively degrade the urban environment. o

%This service is limited by places where cars can traverse so it has varying geographical coverage and big cities such as São Paulo have greater coverage. São Paulo is the richest and a most influential city in Brazil~\cite{ibge2016produto}. There is a high variability in ethnicity and social levels, which contribute to form a multi-cultural city. These facts contribute to the presence of graffiti tagging throughout the city~\cite{theguardian2016pixacao}.

 %is a library of video footage captured by cars driven down the street. The images have been processed to provide panoramic, street-level views of city streets, in which the user can navigate forward or backward along the street, pan 360 degrees, rotate the camera vertically 290 degrees, and zoom in and out (see Figure 1). Google Street View was introduced in 2007 with coverage of a handful of cities but is being extended to new cities at a rapid pace. The image resolution varies depending on when the images were taken, with places photographed more recently being of higher resolution.

%We present a structure-from-motion (SfM) pipeline for visual 3D modeling of a large city area using 360° field of view Google Street View images. The core of the pipeline combines the state of the art techniques such as SURF feature detection, tentative matching by an approximate nearest neighbour search, relative camera motion estimation by solving 5-pt minimal camera pose problem, and sparse bundle adjustment.

% Most relevant to our work
% Snyder touches on a number of larger issues, such as the relationship between graffiti and other criminal activity, the political meaning of graffiti, and ethnographic methods.

%Writers develop graffiti names and styles in an attempt to make a personal mark on the urban landscape

% this book include more thorough discussions about the process and aesthetics of tagging,

%\cite{parra2017automatic}
%\cite{parra2013recognition}
%\cite{schwarzrecognition} recognizes graffiti tags using shape matching. % Database is provided

%EXLAIN ISTANCE SEGMENTATION
% TALK KAIMING HE: MASK RCNN IS SIMPLY FASTER-RCNN + FCN ON EACH ROI
% USE OF PARALLEL HEADS
% ROI pooling may break pixel-to-pixel alignment, so they propose RoiAlign
% META ALGORITHM

% Mask R-CNN [9] extends Faster R-CNN by adding a branch for predicting an object mask in parallel with the existing branch for bounding box recognition.
% Faster R-CNN (Ren et al., 2015) generates region proposals using a region proposal network (RPN), and is currently the leading framework in several object detection bench- marks. Mask R-CNN (He et al., 2017) achieve state-of-the-art performance by adapting Faster R-CNN for instance-level semantic segmentation. In parallel to performing bound- ing box regression and classification, Mask R-CNN additionally predicts a binary object mask. This is different from many other recent systems, in which classification is depen- dent on mask predictions.

% Many recent systems that perform instance-level semantic segmentation make use of the region-based convolutional neural network (R-CNN) object detection framework (Girshick et al., 2014). R-CNN consists of three modules. First, class-agnostic region pro- posals that define the set of candidate detections are generated through selective search (Uijlings et al., 2013). Secondly, a convolutional neural network extracts a fixed-length feature vector for each (warped) region. Lastly, a set of class-specific, linear support vector machines (SVMs) are used for classification. During inference, some 2,000 re- gion proposals are generated. Non-maximum suppression is used to discard sub-optimal bounding boxes, and the SVMs are used to predict the semantic class of each box. Fast R-CNN (Girshick, 2015) makes some modifications to R-CNN that lead to im- provements in terms of both speed and accuracy. DeepMask (Pinheiro et al., 2015) learn to propose candidate object segments, which are then classified by Fast R-CNN. Faster R-CNN (Ren et al., 2015) generates region proposals using a region proposal network (RPN), and is currently the leading framework in several object detection bench- marks. Mask R-CNN (He et al., 2017) achieve state-of-the-art performance by adapting Faster R-CNN for instance-level semantic segmentation. In parallel to performing bound- ing box regression and classification, Mask R-CNN additionally predicts a binary object mask. This is different from

%In addition to cleanup costs, graffiti vandals often shoplift their materials, according to the U.S. Department of Justice. Stealing spray paint and markers adds an additional cost to businesses.

%Vandalism also affects revenue from transportation, as evidenced by the reduction in riders during the 1960s and 1970s. Even before graffiti became associated with gangs, people became afraid of riding the vandalized subways.

%Graffiti sometimes has a wave effect, in which a heavily vandalized area will experience increases in other sorts of crimes as well. Gang-related crimes and violence are the crimes most commonly associated with graffiti.

%Public disorder crimes, such as littering and loitering and other forms of property destruction are sometimes related to graffiti crimes. Because most taggers are males between 15 and 23, there is the concern that tagging may be a "gateway crime," and may lead young offenders to more serious or dangerous crimes such as truancy and drug and alcohol use.

%Vandalism is usually seen as a quality of life issue. When an area has extensive graffiti, people tend to view it as a "bad neighborhood." Nearby property value may decrease and crime may increase. Plus, residents see graffiti as an eyesore. Graffiti that is gang-related or expresses hateful sentiments is most likely to be unwelcome in an area.



==> materials.tex <==

\section{Materials and Methods}

%The description of this work here presented is organized in two sections: image acquisition and graffiti recognition.
In order to confidently estimate the level of graffiti in a geographical region we propose a metric, the \emph{graffiti level}, obtained through the identification and computation of the areas containing graffiti on street view imagery~\cite{googlemaps}.

%###############################
\subsection{Acquisition}
% We use mask rcnn but we do not store the instance segmentation
The region of interest is initially defined and the images are acquired. Due to limitations on the coverage of the pictures provided and on computational constraints, a sample of the full region is considered. There are a number of ways of performing sampling~\cite{stehman1999basic} but they can be classified in random sampling methods and systematic sampling methods. The first removes the bias of the selection by randomly selecting the sample points although not guaranteeing good coverage. The latter, in contrast, assures coverage by including bias.

Once the geographical sample is defined, ideally a full view should be considered for each geographical location. A single $360^{\circ}$ panorama view can be used, but one may need to worry about the distortions present in panoramic photos. Alternatively, complementary views for each location may be considered (see Figure~\ref{fig:views}).

\begin{figure}[h]
        \centering
        \includegraphics[width=0.11\textwidth]{_-235424736_-466441269_0.jpg} 
        \includegraphics[width=0.11\textwidth]{_-235424736_-466441269_90.jpg} 
        \includegraphics[width=0.11\textwidth]{_-235424736_-466441269_180.jpg} 
        \includegraphics[width=0.11\textwidth]{_-235424736_-466441269_270.jpg} 
	\caption{Four views from the same geographical location. Images obtained from~\cite{googlemaps}.}
        \label{fig:views}
\end{figure}

%Discussion on the metric to evalute the level of degradation of a region
%We do not provide google images, but we do provide all the information required to download it from GSV.
 %* How to sample a geographical region? pros/cons
 %* How to handle multiple orientations of the camera? pros/cons

%###############################
\subsection{Graffiti recognition}

Given the objective of quantifying the level of graffiti in a given location, a simple and direct way would be to identify the images containing or not graffiti. Such characterization however give us a sharp and non-precise information of each picture. It would be interesting to have a more granular value for each picture. So we define the graffiti level $G(P)$ of a geographical location $P$ as the total area $A$ of the picture containing graffiti. Such approach can be affected by the projection map of the scene and also by the distance of the camera to the region containing graffiti. We assume that different regions, given a minimum extent, have corresponding distribution of projections and of distance to the walls and with this assumption, $G(P)$ may be used to compare different geographical locations.  Since we represent each location $P$ by a set of $k$ views, we define $G(P)$ as the sum of the areas of the regions containing graffiti in each view (see~(\ref{eq:perphoto})). We can then aggregate the graffiti level by geographical region by computing the average of the graffiti levels on our sample of size $n$ (see~(\ref{eq:perregion})) .

%Since we represent each point by a set of images each representing a view, we .

%\begin{equation}
%	G(P) = \sum_{i=1}^{k} A_i
%	\label{eq:perphoto}
%\end{equation}
%
%\begin{equation}
%	G(R) = \frac{\sum_{j=1}^{n} G(P_j) }{n}
%	\label{eq:perregion}
%\end{equation}

\noindent\begin{minipage}{.34\linewidth}
  \begin{equation}
	G(P) = \sum_{i=1}^{k} A_i
	\label{eq:perphoto}
  \end{equation}
  \end{minipage} \qquad %
\begin{minipage}{.5\linewidth}
  \begin{equation}
	G(R) = \frac{\sum_{j=1}^{n} G(P_j) }{n}
	\label{eq:perregion}
  \end{equation}
  \end{minipage}

%We opted for Mask-RCNN~\cite{he2017mask} method for our segmentation task given its high performance reported on important benchmarks~\cite{cordts2016cityscapes,lin2014microsoft}. Despite it outputs segmentation and instances information, in this work we are just interested on segmentation results.
We opted for Mask-RCNN~\cite{he2017mask} method for our segmentation task given its high performance reported on important benchmarks~\cite{cordts2016cityscapes,lin2014microsoft}. During training, the method minimizes a multi-task loss $L=L_{cls}+L_{box}+L_{mask}$, being the classification loss $L_{cls}$  and bounding-box loss $L_{box}$ the same as defined in~\cite{ren2015faster} and the mask loss $L_{mask}$ defined as the average binary cross-entropy loss. Despite the method outputs segmentation and instance information, in this work we are just interested in the segmentation results.

Since there is no dataset available, we created a dataset with manually annotated images which were used to train our model.

 %* Any scratch on the wall is a graffiti?
 %* Why did I choose mask rcnn?
 %* Is it possible to train a graffiti detector without a training set?
 %* What is image augmentation
 %* How to measure the level of graffiti in an image? pros/cons

%###############################
%\subsection{Case study: São paulo}
%\subsection{Evaluation}
 %* Why Sao Paulo?
 
%We evaluated 
%The most populous city in Latin America.

%Social and economical importance in the country.

%Famous graffiti spots.

% wikimedia commons 
% wall colorful graffiti tags - jwh
% child and guard - Pawel Ryszawa,

% chicao- tags - John H. White, ]
% graffiti wall rose - no author provided
% graffiti wall yellow - agracier

% TODO: Include figure with annotation im_-23.541283999..._-46.6359..._280.jp
%im_-23.54178..._-46.63592...280.jpg

% ##################### Experiments

